The Kummer ratio of the relative class number for prime cyclotomic fields

Kummer's conjecture predicts the asymptotic growth of the relative class number of prime cyclotomic fields. We substantially improve the known bounds of Kummer's ratio under three scenarios: no Siegel zero, presence of Siegel zero and assuming the Riemann Hypothesis for the Dirichlet $L$-series attached to odd characters only. The numerical work in this paper extends and improves on our earlier preprint (arXiv:1908.01152) and demonstrates our theoretical results.

==> Bibliography.tex <==
%{\small
%\begin{thebibliography}{99}

%\bibitem{ABD} A.I. Badzyan,
%The Euler-Kronecker constant,
%\textit{Mat. Zametki}, \textbf{87} (2010), 35--47.

%\bibitem{apos}
%T.M. Apostol, 
%\textit{Introduction to Analytic Number Theory}, Springer-Verlag, 1976.
% thm 13.14


%\bibitem{BJ} %%%not added as it's arxiv
%R. Barbulescu and F. Jouve,
%ECM and the Elliott–Halberstam conjecture for quadratic fields, preprint.
%\ale{\url{https://arxiv.org/pdf/2212.11724.pdf}}
%\ale{The values contained in the table of Example 1, page 18, are not correct.
%Their code (passed me by Barbulescu) produces the correct values instead... 
%(I checked them with my own independently developed program).
%Probably it is just a ``copy-paste'' problem...}

%\bibitem{CM} A. Ciolan, A. Languasco and P. Moree, 
%Landau and Ramanujan approximations for divisor sums and coefficients of cusp forms,
%\textit{J.\,Math.\,Anal.\,Appl.} \textbf{519} (2023), no. 2, Paper No. 126854.

%\bibitem{Dixit} \neelam{A.B. Dixit,
%On Euler-Kronecker constants and the generalized Brauer-Siegel conjecture, 
%\textit{Proc. Amer. Math. Soc.} \textbf{148} (2020), 1399--1414.} 

%\bibitem{DixitMurty} \neelam{A.B. Dixit and M. Ram Murty,
%A localized Erd\H{o}s-Kac theorem for $\omega_y(p + a)$, \textit{Hardy-Ramanujan J.} 
%\textbf{45} (2022), 74--83.} 



%\bibitem{elliot}
%P.D.T.A. Elliott and H. Halberstam, A conjecture in prime number theory.
%\textit{Symp. Math.}, 4 (1968/9), pp. 59--72.


%\bibitem{DixitMurty2} A.B. Dixit and M. Ram Murty, 
%On Ihara's conjectures for Euler-Kronecker constants, \textit{Acta Arith.}, to appear.

%\bibitem{DF} D.S. Dummit and R.M. Foote, 
%\textit{Abstract Algebra}, Prentice Hall, Inc., Englewood Cliffs, NJ, 1991.

%\bibitem{Felix} A.T. Felix, Generalizing the Titchmarsh divisor 
%problem, \textit{Int. J. Number Theory} \textbf{8} (2012), 613--629.

%\bibitem{FLM} K. Ford, F. Luca and P. Moree, Values of the Euler $\phi$-function not divisible by
%a given odd prime, and the distribution of Euler-Kronecker constants for
%cyclotomic fields, \textit{Math. Comp.} \textbf{83} (2014), 1447--1476.

%\bibitem{F} \'E. Fouvry, Sum of Euler-Kronecker constants over consecutive cyclotomic fields, 
%\textit{J. Number Theory} \textbf{133} (2013), 1346--1361.

%\bibitem{FT} A. Fr\"ohlich and M. Taylor, \textit{Algebraic Number Theory}, Cambridge Studies in 
%Advanced Mathematics \textbf{27}, Cambridge University Press, Cambridge, 1993. 

%\bibitem{Gr} A. Granville, On the size of the first factor of the class number
%of a cyclotomic field, \textit{Inv. Math.} \textbf{100} (1990), 321--338.


%\bibitem{Erd} P.~Erd\H os, On a problem of S. Golomb, 
%{\it J. Austral. Math. Soc.} {\bf 2} (1961/1962), 1--8. 

%\bibitem{HL} G.H.~Hardy and J.E.~Littlewood, {\it Some problems of 
%``Partitio Numerorum": III On the expression
%of a number as a sum of primes}, Acta Math. {\bf 44} (1922), 1--70.

%\bibitem{HIKW} Y. Hashimoto,  Y. Iijima, N. Kurokawa and M. Wakayama, Euler's constants for the 
%Selberg and the Dedekind zeta functions, \textit{Bull. Belg. Math. Soc. Simon Stevin} \textbf{11} (2004), 493--516.

%\bibitem{Hasse} H. Hasse, \textit{\"Uber die Klassenzahl Abelscher 
%Zahlk\"orper}, Mathematische Lehrb\"ucher und Monographien, Band I, 
%Berlin, Akademie-Verlag, 1952.

%\bibitem{H1957} \pieter{C. Hooley, On the representation of a number as the sum of two squares and a prime, 
%\textit{Acta Math.} \textbf{97} (1957), 189--210.}

%\bibitem{I} Y. Ihara, On the Euler-Kronecker constants of global fields and primes
%with small norms, \textit{Algebraic Geometry and Number Theory}, 
%Prog. Math. \textbf{253}, 
%Birkh\"auser Boston, Boston, MA, 2006, 407--451.

%\bibitem{I2} Y. Ihara, The Euler-Kronecker invariants in various families of global 
%fields, \textit{Proc. of AGCT 2005} (Arithmetic Geometry and Coding Theory
%10), Ed. F. Rodier et al., S\'eminaires et Congr\`es \textbf{21} (2009), 79--102.

%\bibitem{IMS} Y. Ihara, V. Kumar Murty and M. Shimura, On the 
%logarithmic derivatives of Dirichlet $L$-functions at $s=1$,
%\textit{Acta Arith.} \textbf{137} (2009), 253--276. 

%\bibitem{KLS} N. Kandhil, R. Lunia and J. Sivaraman,
%Explicit upper bounds on the average of Euler-Kronecker constants of narrow 
%ray class fields, preprint.

%\bibitem{KKS} K. Kato, N. Kurokawa and  T. Saito, 
%\textit{Number Theory {\rm 2}. 
%Introduction to Class Field Theory}, 
%Translations of Mathematical Monographs \textbf{240}, Iwanami Series in Modern Mathematics, 
%American Mathematical Society, Providence, RI, 2011.

%\bibitem{Kim}
%\neelam{Henry H. Kim, Extreme values of Euler-Kronecker constants, 
%\textit{Unif. Distrib. Theory}, \textbf{ 16} (2021), 41--52}.

%\bibitem{Kummer} E.E. Kummer, M\'emoire sur la th\'eorie des nombres complexes 
%compos\'ees de racines de l'unit\'e et des nombres entiers, \textit{J. Math. Pures Appl.} \textbf{16} (1851), 
%377--498 (1851); \textit{Collected Works}, Vol. I., pp. 363-484.

%\bibitem{KM} V. Kumar Murty, The Euler-Kronecker constant of a number field, 
%\textit{Ann. Sci.  Math. Qu\'ebec} \textbf{35} (2011), 239--247.

%\bibitem{Lagarias} J.C. Lagarias, Euler's constant: Euler's work and modern developments, 
%\textit{Bull. Amer. Math. Soc.} (N.S.) \textbf{50} (2013), 527--628. 

%\bibitem{Lamzouri2015} Y. Lamzouri, The distribution of Euler-Kronecker constants of quadratic 
%fields,  \textit{J. Math. Anal. Appl.} \textbf{432} (2015), 632--653. 

%\bibitem{c} 
%\ale{Y. Lamzouri,  A. Languasco, 
%\textit{Small values of $\vert L^\prime/L(1,\chi)\vert$}, 
%\newblock {\em Experiment. Math., \textup{\textrm{electronically published on
%  September 3, 2021, DOI:\url{https://doi.org/10.1080/10586458.2021.1927255}
% (to appear in print)}}}, 2021.}
  
  
  
 % \bibitem{murtycojo}
 % M. Ram Murty and A. C. Cojocaru,
 % \textit{An Introduction to Sieve Methods and Their Applications},
%  Cambridge university press,
%  2005.
  
  

%\bibitem{La09a} E. Landau, \textit{L\"osung des Lehmer'schen Problems},
%Amer. J. Math. \textbf{31} (1909), 86--102.

%\bibitem{La09b} E. Landau, \textit{Handbuch der Lehre von der Verteilung
%der Primzahlen}, 3rd ed.,  Chelsea, New York, 1953.

%\bibitem{SL} S. Lang, \textit{Cyclotomic Fields I and II},
%Graduate Texts in Mathematics \textbf{121}, Springer-Verlag, New York, 1990.

%\bibitem{Languasco2021}
%\ale{A. Languasco, Numerical verification of Littlewood's bounds for
%$\vert L(1,\chi)\vert$,  \textit{J. Number Theory} \textbf{223} (2021), 12--34.}

%\bibitem{Languasco2021a}
%\ale{A. Languasco,  
%Efficient computation of the Euler-Kronecker constants for prime cyclotomic fields, 
%\textit{Res. Number Theory} \textbf{7} (2021), Paper n. 2, 1--22.}

%\bibitem{Languasco2023a}
%\ale{A. Languasco,  A unified strategy to compute some special functions
%of number-theoretic interest, 
% \textit{J. Number Theory} \textbf{247} (2023), 118--161.}


%\bibitem{LanguascoR2021}
%\ale{A. Languasco and L. Righi,
%A fast algorithm to compute the {R}amanujan-{D}eninger {G}amma
%function and some number-theoretic applications,
%\textit{Math. Comp.} \textbf{90} (2021), 2899--2921.}

%\bibitem{Linnik} Yu. V. Linnik, \textit{The Dispersion Method in Binary Additive Problems}, 
%Transl. Math. Monographs \textbf{4}, Amer. Math. Soc., Providence, Rhode Island, 1963.

%\bibitem{Marcus} D. Marcus, \textit{Number Fields}, Universitext, Springer-Verlag, 
%New York-Heidelberg, 1977. 

%\bibitem{MaMo} \pieter{L.\,Martirosyan and P.\,Moree,
%Large absolute values of cyclotomic polynomials at roots of unity, 
%\textit{J. Number Theory} \textbf{239} (2022), 251--272.}

%\bibitem{MVsieve} H.L. Montgomery and R.C. Vaughan, The large sieve, 
%\textit{Mathematika} \textbf{20} (1973), 119--134. 

%\bibitem{MV} H.L. Montgomery and R.C. Vaughan,
%\textit{Multiplicative Number Theory I. Classical Theory}, Cambridge studies in
%advanced mathematics vol. 97, Cambridge University Press, 2007.

%\bibitem{MIndia} P. Moree, Counting numbers in multiplicative sets: Landau versus Ramanujan,
%\textit{Mathematics Newsletter} \textbf{21}, no. 3 (2011), 73--81 (arXiv:1110.0708).


%\bibitem{MSurvey} P. Moree, Irregular behaviour of class numbers and
%Euler-Kronecker constants of cyclotomic fields: the log log log devil at play,
%in `\textit{Irregularities in the Distribution of Prime Numbers - Research Inspired
%by Maier's Matrix Method}', Eds. J. Pintz and M. Th. Rassias, Springer, 2018, 143--163.

%\bibitem{MZ} M.R. Murty and A. Zaytseva, Transcendence of generalized Euler constants, 
%\textit{Amer. Math. Monthly} \textbf{120} (2013), 48--54. 

%\bibitem{MM}
%\neelam{M. Mourtada and V. Kumar Murty,
%Omega theorems for $\frac{L'}{L}(1,\chi_D)$, \textit{Int. J. Number Theory,}
%\textbf{9} (2013), 561--581.}

%\bibitem{MM2}
%\neelam{M. Mourtada and V. Kumar Murty,
%On the Euler-Kronecker constant of a cyclotomic field, II, \textit{Contemporary Mathematics,}
%\textbf{ 655} (2015), 143--151.

%\bibitem{murtyy}
%M. Ram Murty,
%\textit{Problems in analytic number theory},
%Springer.

%\bibitem{MP} M. Ram Murty and Y.N. Petridis, On Kummer's 
%conjecture, \textit{J. Number Theory} \textbf{90} (2001), 294--303. 

%\bibitem{N} W. Narkiewicz, \textit{Elementary and Analytic Theory of Algebraic Numbers}. Second edition. 
%Springer-Verlag, Berlin; PWN---Polish Scientific Publishers, Warsaw, 1990.

%\bibitem{Prachar} 
%K. Prachar, 
%\textit{Primzahlverteilung}, Reprint of the 1957 original, Grundlehren der Mathematischen Wissenschaften \textbf{91}, Springer-Verlag, Berlin-New York, 1978. 

%\bibitem{Olivier} O. Ramar\'e, \textit{Arithmetical Aspects of the Large Sieve Inequality}, 
%With the collaboration of D.S. Ramana, Harish-Chandra Research Institute Lecture Notes 
%\textbf{1}, Hindustan Book Agency, New Delhi, 2009.

%\bibitem{T} M.A. Tsfasman, Asymptotic behaviour of the Euler-Kronecker constant, in 
%V. Ginzburg, ed., \textit{Algebraic Geometry and Number Theory: In Honor of Vladimir 
%Drinfeld's 50th Birthday}, Progress in Mathematics, Vol. 850, 
%Birkh\"auser Boston, Cambridge, MA, 2006, 453--458.

%\bibitem{Washington} L.C. Washington, \textit{Introduction to Cyclotomic Fields}, Graduate Texts in Mathematics \textbf{83}, Springer-Verlag, 
%New York, 1982.

%\bibitem{Washington} L.C. Washington, 
%\textit{Introduction to Cyclotomic Fields}, Second edition, Graduate Texts in 
%Mathematics \textbf{83}, Springer-Verlag, New York, 1997.

%\bibitem{zykin} \neelam{A. Zykin,
%Asymptotic properties of Dedekind zeta functions in families of number fields, 
%\textit{Journal de Théorie des Nombres de Bordeaux},
%\textbf{22} (2010), 771--778.}

%\bibitem{zykin2} \neelam{A. Zykin,
%Asymptotic properties of zeta functions over
%finite fields, \textit{Finite fields and their applications}, \textbf{35} (2015), 247--283.}


%\end{thebibliography}}
